Sparsity of Fourier mass of passively advected scalars in the Batchelor regime

In 1959, Batchelor gave a prediction for the power spectral density of a passive scalar advected by an incompressible fluid exhibiting shear-straining, a mechanism for the creation of small scales in the scalar [Bat59]. Recently, a `cumulative' version of this law, summing over Fourier modes below a given wavenumber $N$, was given for a broad class of passive scalars under incompressible advection, including by solutions to the stochastic Navier-Stokes equations [BBPS22c]. This paper addresses to what extent Fourier mass of such passive scalars truly saturates the predicted power law scaling due to Batchelor. Via discrete-time pulsed-diffusion models of the advection-reaction equations, we exhibit situations compatible with the cumulative law but for which the distribution of Fourier mass among wavenumbers $|k| \leq N$ is relatively \emph{sparse} and much smaller than a `mode-wise' version of Batchelor's original prediction. In the same situations we also establish an `exponential radial shell' version of Batchelor's laws via a novel application of the method of spectral distributions.

==> conclusion.tex <==
%!TEX root = main.tex


\subsection*{Sparsity}
\begin{itemize}
    \item angular sparsity for standard map in discrete time or Pierrehumbert in continuous time
    \item can you build a better model which exhibits pulse localization like in section 4? 
\end{itemize}

\subsection*{Non-sparsity results}
\begin{itemize}
    \item can one prove an exponential shell law is valid for `general' systems? 
    \item what we can show: assumptions of section 2 imply exponential shell-based upper bound $\lesssim (\frac{1}{\gamma} - \frac{1}{\lambda}) \log N$. 
    \item proof in appendix
    \item proof of exponential shell law will require ruling out cancellations from superposition of multiple pulses. could be subtle.
    \item {\color{red} when the cat map randomly alternates between two general matrices, we could have angular non-sparsity results}
\end{itemize}

\subsection*{Role of dynamical systems tools in the Batchelor regime}

One possiblity: use ruelle resonances, a.k.a. strange eigenmodes: 

\begin{itemize}
    \item conditional theorem: if $\Lc_f$ admits a norm with spectral gap and dominant eigendistribution $\psi_f$, then stationary PSA are norm-close to the span of $\psi_f$ (away from some integral range depending on the forcing term). 
    \item this is an ultimate kind of `sparsity': concentration of stationary mass along a one-dimensional line in some negative sobolev space 
    \item of interest to develop this further for nonautonomous flows. big open frontier. 
\end{itemize}

{\color{red} {Another possiblity: use countable Lebesgue spectrum. This suggests a strong sparsity!!!
}
  } 


% some open questions: 
% \begin{itemize}
%     \item would be nice to treat a system coming from a time-periodic flow, e.g., the piecewise linear model put forward in [Elgindi-Liss-Mattingly]. how to deal with singularity curves? there are parameter regions for their system for which the stable directions are more or less aligned completely. issue now is that the singularities introduce lots of fine scales jumping around all over the place. perhaps Fourier is a bad basis for measuring? 
%     \item what happens if you use different orthonormal basis than fourier? comment on Lebesgue spectrum for dynamical systems - would be exactly this `pulses' business. now one deals with the interaction between this `funny', generally low-regularity basis and the heat kernel coming from the original system. what happens here? 
% \end{itemize}



==> cumLaw.tex <==
%!TEX root = main.tex



{\bf potentially delete? }

\subsection{Cumulative upper bound}
\begin{lemma}[Cumulative law's upper bound:]

For any $N\geq3$ we have 
\end{lemma}

\begin{equation}
\mathbb{E}\sum_{\left|k\right|\leq N}\left|\widehat{g_{\mathrm{stat}}^{a,\kappa}}\left(k\right)\right|^{2}=\mathbb{E}\left\Vert P_{\leq N}g_{\mathrm{stat}}^{a,\kappa}\right\Vert _{L^{2}\left(\mathbb{T}^{2}\right)}^{2}\lesssim_{\neg\kappa,\neg a,\tilde{a}}\ln N\label{eq:upper_inertial}
\end{equation}

\begin{proof}
By Ito isometry / Pythagoras:
\begin{align}
A_{m}:=\mathbb{E}\left\Vert P_{\leq N}\sum_{n=0}^{m}\eta_{n}\mathcal{L}_{\kappa,f_{a}}^{n}e_{k_{0}}\right\Vert _{L^{2}}^{2} & \stackrel{``isometry"}{=}\sum_{n=0}^{m}\mathbb{E}\left\Vert \eta_{n}P_{\leq N}\mathcal{L}_{\kappa,f_{a}}^{n}e_{k_{0}}\right\Vert _{L^{2}}^{2}\nonumber \\
 & =\sum_{n=0}^{m}\left\Vert P_{\leq N}\mathcal{L}_{\kappa,f_{a}}^{n}e_{k_{0}}\right\Vert _{L^{2}}^{2}\label{eq:isometry_ito-1}
\end{align}
Recall that $\left\Vert .\right\Vert _{H^{-p}}\leq\left\Vert .\right\Vert _{\mathrm{CAT}}$.
We have late-time control with Bernstein and exponential mixing \eqref{eq:contraction_kappa}:
\begin{align*}
\left\Vert P_{\leq N}\mathcal{L}_{\kappa,f_{a}}^{n}e_{k_{0}}\right\Vert _{L^{2}}^{2} & \lesssim N^{2p}\left\Vert P_{\leq N}\mathcal{L}_{\kappa,f_{a}}^{n}e_{k_{0}}\right\Vert _{H^{-p}}^{2}\lesssim N^{2p}\left\Vert \mathcal{L}_{\kappa,f_{a}}^{n}e_{k_{0}}\right\Vert _{\mathrm{CAT}}^{2}\lesssim_{\tilde{a}}N^{2p}e^{-2n\widetilde{\gamma}}
\end{align*}
and early-time control (which is the late-time portion in Batchelor
paper)
\begin{align*}
\left\Vert P_{\leq N}\mathcal{L}_{\kappa,f_{a}}^{n}e_{k_{0}}\right\Vert _{L^{2}}^{2} & \lesssim1
\end{align*}

So we conclude
\begin{align*}
\mathbb{E}\left\Vert P_{\leq N}g_{\mathrm{stat}}^{a,\kappa}\right\Vert _{L^{2}}^{2}=\limsup_{m\to\infty}A_{m} & \lesssim\sum_{n=0}^{m}\min\left(N^{2p}e^{-n\widetilde{\gamma}},1\right)=\sum_{n=0}^{\left\lfloor 2p\widetilde{\gamma}^{-1}\ln N\right\rfloor }1+\sum_{n=\left\lceil 2p\tilde{\gamma}^{-1}\ln N\right\rceil }^{m}N^{2p}e^{-2n\widetilde{\gamma}}\\
 & \lesssim2p\tilde{\gamma}^{-1}\ln N+N^{2p}\cdot N^{-2p}\lesssim_{p,\tilde{\gamma}}\ln N
\end{align*}
\end{proof}
It is easier to work directly with $g_{\mathrm{stat}}^{a,\kappa}$,
unlike in the Batchelor paper \cite{bedrossianBatchelorSpectrumPassive2020}
where we would need Birkhoff ergodic theorem.

The cumulative upper bound
\[
\sum_{\left|k\right|\leq N}\left|\widehat{\phi}\left(k\right)\right|^{2}\lesssim\ln N
\]
 implies $\sum_{N<\left|k\right|\leq2N}\left|\widehat{\phi}\left(k\right)\right|^{2}\lesssim\ln N$
which implies $\phi\in H^{0-}.$ So $g_{\mathrm{stat}}^{a,\kappa}$
is $H^{0-}$-valued. However, when $\kappa>0$, we can show $g_{\mathrm{stat}}^{a,\kappa}$
is $L^{2}$-valued, as is done next.

\subsection{Energy balance law and upper bound in dissipative range}

% Preview source code from paragraph 69 to 75

We recall the simple inequality 
\[
\left\Vert e^{-\kappa\Lambda^{2}}\phi\right\Vert _{H^{s}}\leq e^{-\kappa}\left\Vert \phi\right\Vert _{H^{s}}
\]
for any $s\geq0$ and $\phi\in H^{s}$ such that $\widehat{\phi}\left(0\right)=0$.

Let $\Phi=g_{\mathrm{stat}}^{a,\kappa}$ which is $\mathrm{CAT}_{0}$-valued.
Then by the independence of $\left(\eta_{n}\right)_{n\in\mathbb{N}}$
and the fact that $\left\Vert \mathcal{L}_{f_{a}}\phi\right\Vert _{L^{2}}=\left\Vert \phi\right\Vert _{L^{2}}\;\forall\phi\in L^{2}$:
\[
\mathbb{E}\left\Vert \Phi\right\Vert _{L^{2}}^{2}=\sum_{n\in\mathbb{N}}\left\Vert \left(e^{-\kappa\Lambda^{2}}\mathcal{L}_{f_{a}}\right)^{n}e_{k_{0}}\right\Vert _{L^{2}}^{2}\leq\sum_{n\in\mathbb{N}}e^{-\kappa n}<\infty
\]
for any $\kappa<0$. Which implies that $\Phi$ as a random variable
is $L^{2}$-valued.

Let $\omega_{*}=\eta_{*}e_{k_{0}}$ be an IID copy of any $\omega_{n}=\eta_{n}e_{k_{0}}$.
We have the energy balance equation (between dissipation from heat
and gain from noise) 
\begin{align}
\mathbb{E}\left\Vert \Phi\right\Vert _{L^{2}}^{2} & =\mathbb{E}\left\Vert e^{-\kappa\Lambda^{2}}\mathcal{L}_{f_{a}}\Phi+\eta_{*}e_{k_{0}}\right\Vert _{L^{2}}^{2}\label{eq:independence_trick}\\
 & =\mathbb{E}\left\Vert e^{-\kappa\Lambda^{2}}\mathcal{L}_{f_{a}}\Phi\right\Vert _{L^{2}}^{2}+\mathbb{E}\left|\eta_{*}\right|^{2}\left\Vert e_{k_{0}}\right\Vert _{L^{2}}^{2}\nonumber \\
 & =\mathbb{E}\left\Vert e^{-\kappa\Lambda^{2}}\mathcal{L}_{f_{a}}\Phi\right\Vert _{L^{2}}^{2}+1\nonumber 
\end{align}

Since $\left\Vert \Phi\right\Vert _{L^{2}}^{2}=\left\Vert \mathcal{L}_{f_{a}}\Phi\right\Vert _{L^{2}}^{2}$,
this implies 
\begin{align}
1 & =\mathbb{E}\left\Vert \mathcal{L}_{f_{a}}\Phi\right\Vert _{L^{2}}^{2}-\mathbb{E}\left\Vert e^{-\kappa\Lambda^{2}}\mathcal{L}_{f_{a}}\Phi\right\Vert _{L^{2}}^{2}=\mathbb{E}\sum_{k\neq0}\left|\widehat{\mathcal{L}_{f_{a}}\Phi}\left(k\right)\right|^{2}-\mathbb{E}\sum_{k\neq0}e^{-\kappa\left|k\right|^{2}}\left|\widehat{\mathcal{L}_{f_{a}}\Phi}\left(k\right)\right|^{2}\nonumber \\
 & =\mathbb{E}\sum_{k\neq0}\left(1-e^{-\kappa\left|A^{-T}k\right|^{2}}\right)\left|\widehat{\mathcal{L}_{f_{a}}\Phi}\left(k\right)\right|^{2}\gtrsim\mathbb{E}\sum_{k\neq0}\kappa\left|k\right|^{2}e^{-\kappa\left|A^{-T}k\right|^{2}}\left|\widehat{\mathcal{L}_{f_{a}}\Phi}\left(k\right)\right|^{2}\nonumber \\
 & =\kappa\mathbb{E}\left\Vert e^{-\kappa\Lambda^{2}}\mathcal{L}_{f_{a}}\Phi\right\Vert _{H^{1}}^{2}\label{eq:kappa_balance}
\end{align}

which is analogous to the $L^{2}$ balance equation (Equation (1.4) in \cite{bedrossian2022batchelor}).
This also implies $\mathbb{E}\left\Vert e^{-\kappa\Lambda^{2}}\mathcal{L}_{f_{a}}\Phi\right\Vert _{H^{1}}^{2}\lesssim\frac{1}{\kappa}$
and similar to \eqref{eq:independence_trick}, we have
\[
\mathbb{E}\left\Vert \Phi\right\Vert _{H^{1}}^{2}=\mathbb{E}\left\Vert e^{-\kappa\Lambda^{2}}\mathcal{L}_{f_{a}}\Phi+\eta_{*}e_{k_{0}}\right\Vert _{H^{1}}^{2}=\mathbb{E}\left\Vert e^{-\kappa\Lambda^{2}}\mathcal{L}_{f_{a}}\Phi\right\Vert _{H^{1}}^{2}+1\lesssim\frac{1}{\kappa}+1
\]

Consequently, combining with the cumulative upper bound \eqref{eq:upper_inertial},
for $\kappa>0$ small we have
\begin{align*}
\mathbb{E}\left\Vert g_{\mathrm{stat}}^{a,\kappa}\right\Vert _{L^{2}}^{2} & \leq\mathbb{E}\left\Vert P_{\leq\frac{1}{\sqrt{\kappa}}}\Phi\right\Vert _{L^{2}}^{2}+\mathbb{E}\left\Vert P_{>\frac{1}{\sqrt{\kappa}}}\Phi\right\Vert _{L^{2}}^{2}\\
 & \lesssim\left|\ln\kappa\right|+\kappa\mathbb{E}\left\Vert P_{>\frac{1}{\sqrt{\kappa}}}\Phi\right\Vert _{H^{1}}^{2}\\
 & \lesssim_{\tilde{a}}\left|\ln\kappa\right|+1
\end{align*}



\subsection{Cumulative lower bound}

We observe that $\forall\phi\in H^{1}:$
\begin{align*}
\left\Vert \mathcal{L}_{f}\phi\right\Vert _{H^{1}}^{2} & \sim_{\lambda}\left\Vert \phi\right\Vert _{H^{1}}^{2}\\
\implies\left\Vert \mathcal{L}_{f_{a}}\phi\right\Vert _{H^{1}}^{2} & \sim_{\lambda,\tilde{a}}\left\Vert \phi\right\Vert _{H^{1}}^{2}
\end{align*}
for {\mbox{$\widetilde{a}$} small enough}.
\begin{claim}
Now we show the lower bound: 
\[
\mathbb{E}\sum_{\left|k\right|\leq N}\left|\widehat{g_{\mathrm{stat}}^{a,\kappa}}\left(k\right)\right|^{2}\gtrsim\ln N
\]
for all $N\in\left[N_{0},\kappa^{-\frac{1}{2}}\right]$.
\end{claim}

\begin{proof}
Fix $\vartheta>0$ (to be chosen later). We simply estimate the early-time
portion. We have from \eqref{eq:isometry_ito-1}: 
\begin{align}
\mathbb{E}\sum_{\left|k\right|\leq N}\left|\widehat{g_{\mathrm{stat}}^{a,\kappa}}\left(k\right)\right|^{2} & =\liminf_{m\to\infty}\sum_{n=0}^{m}\left\Vert P_{\leq N}\mathcal{L}_{\kappa,f_{a}}^{n}e_{k_{0}}\right\Vert _{L^{2}}^{2}\geq\sum_{n=0}^{\vartheta\ln N}\left\Vert P_{\leq N}\mathcal{L}_{\kappa,f_{a}}^{n}e_{k_{0}}\right\Vert _{L^{2}}^{2}\\
 & =\sum_{n=0}^{\vartheta\ln N}\left\Vert \mathcal{L}_{\kappa,f_{a}}^{n}e_{k_{0}}\right\Vert _{L^{2}}^{2}-\sum_{n=0}^{\vartheta\ln N}\left\Vert P_{>N}\mathcal{L}_{\kappa,f_{a}}^{n}e_{k_{0}}\right\Vert _{L^{2}}^{2} 
\end{align}


We first deal with the high-frequency term. Recall that $\left\Vert \mathcal{L}_{\kappa,f_{a}}\phi\right\Vert _{H^{1}}\leq e^{C_{1}}\left\Vert \phi\right\Vert _{H^{1}}$for
some $C_{1}>0$ depending on $\widetilde{a}$.

And therefore
\begin{align*}
\sum_{n=0}^{\vartheta\ln N}\left\Vert P_{>N}\mathcal{L}_{\kappa,f_{a}}^{n}e_{k_{0}}\right\Vert _{L^{2}}^{2} & \lesssim N^{-2}\sum_{n=0}^{\vartheta\ln N}\left\Vert \mathcal{L}_{\kappa,f_{a}}^{n}e_{k_{0}}\right\Vert _{H^{1}}^{2}\\
 & \lesssim N^{-2}\sum_{n=0}^{\vartheta\ln N}e^{C_{1}n}\\
 & \lesssim_{\neg\vartheta}N^{C_{1}\vartheta-2}
\end{align*}
{Pick \mbox{$\vartheta$} small} so that $C_{1}\vartheta\ll2$
and $\sum_{n=0}^{\vartheta\ln N}\left\Vert P_{>N}\mathcal{L}_{\kappa,f_{a}}^{n}e_{k_{0}}\right\Vert _{L^{2}}^{2}<\frac{1}{4}$.

Then for the full-frequency term: let $\phi_{n}=\mathcal{L}_{\kappa,f_{a}}^{n}e_{k_{0}}$.
Then similar to the Fourier argument in \eqref{eq:kappa_balance},
we have 
\[
\left\Vert \phi_{n}\right\Vert _{L^{2}}^{2}-\left\Vert \phi_{n+1}\right\Vert _{L^{2}}^{2}=O\left(\kappa\right)\left\Vert \mathcal{L}_{f_{a}}\phi_{n}\right\Vert _{H^{1}}^{2}\leq O\left(\kappa\right)e^{2C_{1}}\left\Vert \phi_{n}\right\Vert _{H^{1}}^{2}\lesssim_{\neg n}\kappa e^{2C_{1}\left(n+1\right)}
\]
which implies 
\[
\underbrace{\left\Vert \phi_{0}\right\Vert _{L^{2}}^{2}}_{1}-\left\Vert \phi_{n}\right\Vert _{L^{2}}^{2}\lesssim_{\neg n}\kappa\sum_{k=0}^{n}e^{2C_{1}k}\lesssim_{\neg n}\kappa e^{2C_{1}n}
\]

For all $n<\vartheta\ln N$ with {\mbox{$\vartheta$} small
enough}, we will have $1-\left\Vert \phi_{n}\right\Vert _{L^{2}}^{2}<\frac{1}{4}$. 

Therefore:
\[
\sum_{n=0}^{\vartheta\ln N}\left\Vert \mathcal{L}_{\kappa,f_{a}}^{n}e_{k_{0}}\right\Vert _{L^{2}}^{2}\geq\frac{3}{4}\left(\vartheta\ln N\right)-\frac{1}{4}\gtrsim\ln N.
\]
\end{proof}

==> microlocal.tex <==
%!TEX root = main.tex

\subsection{Preliminaries on pseudodifferential operators on manifolds}

\begin{itemize}
    \item following Faure; see also ... for alternative treatments
    \item Let $M$ be a smooth compact Riemannian manifold without boundary, and $TM, T^* M$ the tangent and cotangent bundles respectively. 
    \item fix cutoff $\chi : TM \to [0,1]$ supported in a neighborhood $U$ of the zero section $\mathbf{0}$ along which the exponential map $\exp_x$ is injective for each $U_x := U \cap T_x M$. 
    \item \begin{definition}
        \begin{itemize}
            \item symbol $a(x, \xi)$
            \item pseudodifferential operator $\hat a$ associated to $a$
        \end{itemize}
    \end{definition}
    \item of interest are the class of PDO's with symbols 
    \[A_m(x, \xi) = \langle \xi \rangle^{m(x, \xi)}\]
    where $m : T^* M \to \R$ is a smooth function depending only on the projective direction of $\xi$, i.e., 
    \[m(x, \xi) = m(x, \xi / |\xi|) \, , \]
    where we abuse notation somewhat and write $|\cdot|$ for the metric length in $T^*_x M$. 
    \item observation: given $m$ bounded and smooth as above, $\hat A_m$ is invertible and formally self-adjoint. Definition of $H^m$, duality with $H^{-m}$ through $L^2$ pairing. 
\end{itemize}

\subsection{Anisotropic spaces for uniformly hyperbolic maps}

\begin{itemize}
    
    \item \begin{definition}
        uniformly hyperbolic map
    \end{definition}
    \item Conditions on the order function: 
    \begin{itemize}
        \item \[m \circ F - m \leq - c < 0 \, , \]   
        \item $m \equiv u > 0$ near $E^u$, $m \equiv -s < 0$ near $E^s$, and $-s \leq m \leq u$ pointwise elsewhere. 
    \end{itemize}
    
    \item Theorem (just state it): Compact + Small (as in Section 3)
    \item special case: CAT map. 
\end{itemize}


\subsection{Proof of Proposition ???}

\begin{itemize}
    \item Proof here of equivalence between anisotropic norms a la Faure with those in Section 3. 
    
\end{itemize}


\section{Faure-Sjöstrand microlocal approach}

% Preview source code from paragraph 127 to 241


Ruelle transfer operator 
\[
\hat{F}\phi=\phi\circ f
\]

Simple observation: hyperbolic $\implies$ high Fourier modes of $\hat{F}^{n}\phi$
go to infinity as $n\to\pm\infty$. In other words, energy cascade
towards fine scales, decay of correlation. Ruelle resonances govern
the exponential decay. Later improved by Keller-Liverani: Ruelle resonances
are discrete spectrum of transfer operator (in some function space).
Also linked to escape of quantum wave function in open quantum systems
(light emission, radioactive decay).

In semi-classical / microlocal analysis we are concerned with PDO
and FIO
\begin{enumerate}
\item Pseudo-differential operator: to each PDO $\widehat{P}$ we have a
\textbf{symbol} function $P=\sigma\left(\widehat{P}\right)$ on $T^{*}M$.
\item Fourier integral operator: to each FIO $\widehat{F}$ we have a symplectic
map $F$ on $T^{*}M$. 
\begin{itemize}
\item \textbf{Ruelle transfer operator} $\widehat{F}$ is FIO where $F:T^{*}M\to T^{*}M$
is lift of $f^{-1}$, where $f$ is Anosov diffeo.
\begin{itemize}
\item Trajectories are non-compact except section $\xi=0$. Leading to discreteness
of spectrum. We construct \emph{escape function} $A_{m}$ that decreases
along non-compact trajectories (decreasing in unstable direction,
increasing in stable direction). Let $\widehat{A_{m}}$ be associated
invertible PDO. We get anisotropic Sobolev 
\[
H^{m}=\widehat{A_{m}}^{-1}\left(L^{2}\left(M\right)\right)
\]
Outside arbitrarily small disk $B\left(0,\epsilon_{m}\right)$, $\widehat{F}$
has discrete spectrum which \uline{does not depend on choice} of $A_{m}$,
and this defines Ruelle resonances. We mainly use: 
\begin{enumerate}
\item composition of PDO, 
\item Egorov's transport theorem
\item $L^{2}$ continuity theorem.
\end{enumerate}
\end{itemize}
\end{itemize}
\end{enumerate}

\subsection{Setting \protect\label{subsec:Setting}}
\begin{itemize}
\item Let $M$ be smooth, compact, connected manifold (like torus).
\item Let $f:M\to M$ be $C^{\infty}$ \textbf{Anosov diffeomorphism}. In
other words, there is Holder-continuous Riemannian metric $g_{0}$
(\textbf{Lyapunov metric}) and an $f$-\textbf{invariant} orthogonal
decomposition 
\begin{equation}
TM=E_{u}\oplus E_{s}\label{eq:anosov_decomp}
\end{equation}
with $\theta\in\left(0,1\right)$ such that:
\begin{align*}
\left|D_{x}f\left(v_{s}\right)\right|_{g_{0}} & \leq\theta\left|v_{s}\right|_{g_{0}}\;\forall x\in M,v_{s}\in E_{s}\left(x\right)\\
\left|D_{x}f^{-1}\left(v_{u}\right)\right|_{g_{0}} & \leq\theta\left|v_{u}\right|_{g_{0}}\;\forall x\in M,v_{u}\in E_{u}\left(x\right)
\end{align*}

\begin{itemize}
\item Example: hyperbolic automorphism of $\mathbb{T}^{n}$ and $C^{1}$-small
perturbation by \textbf{structural stability theorem} \parencite[Corollary 6.4.7, page 266]{katokIntroductionModernTheory1995}:
any $C^{1}$ small perturbation of Anosov diffeo is Anosov.
\item Need to smoothen $g_{0}$: Let $g$ be smooth such that $\exists c\in\left[1,\frac{1}{\sqrt{\theta}}\right):\frac{1}{c}g_{0}\leq g\leq cg_{0}$.
This implies 
\begin{align}
\left|D_{x}f\left(v_{s}\right)\right|_{g} & \leq c^{2}\theta\left|v_{s}\right|_{g_{0}}\;\forall x\in M,v_{s}\in E_{s}\left(x\right)\nonumber \\
\left|D_{x}f^{-1}\left(v_{u}\right)\right|_{g} & \leq c^{2}\theta\left|v_{u}\right|_{g_{0}}\;\forall x\in M,v_{u}\in E_{u}\left(x\right)\label{eq:smoothened}
\end{align}
We will always work with smoothened metric $g$. \textcolor{red}{But
does it still preserve orthogonality like g?}
\end{itemize}
\item With $f$ and $M$ as above, define an arbitrary smooth density $dx=d\mu_{\mathrm{Leb}}$
such that $\mu_{\mathrm{Leb}}\left(M\right)=1$.
\item \textbf{Ruelle transfer operator} $\widehat{F}\phi=\phi\circ f$ for
any $\phi\in L^{2}\left(M\right)$.
\begin{itemize}
\item Could also consider $\widehat{F}\phi=\phi\circ f^{-1}$. Just up to
convention.
\item If $f$ preserves $\mu_{\mathrm{Leb}}$ then $\widehat{F}$ is unitary
on $L^{2}$.
\item Adjoint of $\widehat{F}$ is \textbf{Perron-Frobenius operator} 
\[
\left(\widehat{F}^{*}\phi\right)\left(y\right)=\frac{\phi\left(f^{-1}y\right)}{\left|\det D_{f^{-1}y}f\right|}\;\forall\phi\in C^{\infty}\left(M\right)
\]
\item Another type of transfer operator in Ruelle's thermodynamic formalism
is 
\[
\widehat{F}_{V}\phi\left(x\right)=\phi\left(f\left(x\right)\right)e^{V\left(x\right)}
\]
where $V\in C^{\infty}\left(M\right)$ is a potential. This is a special
case of transfer operators acting on sections of line bundles (used
in quantum chaos and geometric quantization).
\end{itemize}
\item Lift $f^{-1}$ to $F=T^{*}f^{-1}$
\begin{align*}
F:T_{x}^{*}M & \to T_{f^{-1}x}^{*}M\\
\xi & \mapsto\xi\circ\left(D_{f^{-1}x}f\right)=\left(D_{f^{-1}x}f\right)^{t}\xi
\end{align*}
So $F\xi:T_{f^{-1}x}M\xrightarrow{\left(D_{f^{-1}x}f\right)}T_{x}M\xrightarrow{\xi}\mathbb{R}.$ 
\begin{itemize}
\item In microlocal analysis, $F$ is the canonical symplectic map associated
to the FIO $\widehat{F}$. This appears in Egorov's theorem.
\item Let $T^{*}M=E_{s}^{*}\oplus E_{u}^{*}$ being the \textbf{decomposition
dual} of \eqref{eq:anosov_decomp}, i.e. $E_{s}^{*}\left(E_{u}\right)=0,E_{u}^{*}\left(E_{s}\right)=0$.
We have the dual of \eqref{eq:smoothened}
\begin{align}
\left|F\left(\xi_{s}\right)\right|_{g}=\left|T^{*}\left(f^{-1}\right)\xi_{s}\right|_{g} & \leq c^{2}\theta\left|\xi_{s}\right|_{g}\;\forall x\in M,\xi_{s}\in E_{s}^{*}\left(x\right)\nonumber \\
\left|F\left(\xi_{u}\right)\right|_{g}=\left|T^{*}\left(f^{-1}\right)\xi_{u}\right|_{g} & \leq c^{2}\theta\left|\xi_{u}\right|_{g}\;\forall x\in M,\xi_{u}\in E_{u}^{*}\left(x\right)\label{eq:smoothened-1}
\end{align}
\end{itemize}
\end{itemize}

\subsection{Microlocal analysis}

\subsubsection{Summary of traditional microlocal}

For a smooth \textbf{symbol} function $P\left(x,\xi\right)$ with
conditions at infinity we have PDO $\widehat{P}$
\begin{equation}
\widehat{P}\phi\left(x\right)=\int_{\mathbb{R}^{2d}}P\left(x,\xi\right)\phi\left(y\right)e^{i2\pi\xi\left(x-y\right)}\;dyd\xi\label{eq:PDO}
\end{equation}

In particular, with $\widehat{P}=\left(\frac{D}{i2\pi}\right)^{\alpha}$
we have 
\[
\left(\frac{D}{i2\pi}\right)^{\alpha}\phi\left(x\right)=\int_{\mathbb{R}^{d}}\xi^{\alpha}\widehat{\phi}\left(\xi\right)e^{i2\pi\xi x}\;d\xi=\int_{\mathbb{R}^{2d}}\xi^{\alpha}\phi\left(y\right)e^{i2\pi\xi\left(x-y\right)}\;dyd\xi
\]
So PDO includes ordinary differential operators. On the other hand
with $\psi\left(x\right)\in\mathcal{S}\left(R^{d}\right)$ we have
\[
\psi\left(x\right)\phi\left(x\right)=\phi\left(x\right)\int_{\mathbb{R}^{d}}\widehat{\phi}\left(\xi\right)e^{i2\pi\xi x}\;d\xi=\int_{\mathbb{R}^{2d}}\psi\left(x\right)\phi\left(y\right)e^{i2\pi\xi\left(x-y\right)}\;dyd\xi
\]
so with the symbol $p\left(x,\xi\right)=\psi\left(x\right)$ we have
the zero-order PDO $M_{\psi}\phi=\psi\phi$ (not smoothing operator).

We have three main results
\begin{enumerate}
\item Composition of PDO by principal symbols: $\sigma_{\mathrm{prin}}\left(\hat{P}\right)\sigma_{\mathrm{prin}}\left(\widehat{Q}\right)=\sigma_{\mathrm{prin}}\left(\hat{P}\hat{Q}\right)$.
\item Sobolev continuity: a PDO $\widehat{P}$ maps $H^{s}\to H^{s-m}$
continuously depending on the symbol.
\item Ellipticity + parametrix: an ellipticity condition on symbol ensures
PDO is invertible modulo some regularization. The ``almost-inverse''
is called a parametrix.
\end{enumerate}
\begin{itemize}
\item We define the symbol class of \emph{constant order} $S_{\rho,\delta}^{m}\subseteq C^{\infty}\left(\mathbb{R}^{2n}\right)$
($m,\rho,\delta\in\mathbb{R}$) which includes smooth functions $P\left(x,\xi\right)$
which satisfies 
\[
\left|\partial_{\xi}^{\alpha}\partial_{x}^{\beta}P\left(x,\xi\right)\right|\lesssim_{K,\alpha,\beta}\left\langle \xi\right\rangle ^{m-\rho\left|\alpha\right|+\delta\left|\beta\right|}\;\forall x\in K\text{ compact}
\]

\begin{itemize}
\item Example: with $\widehat{P}=\left(\frac{D}{i2\pi}\right)^{\alpha},P=\xi^{\alpha}$
and $\left|\partial_{\xi}^{\widetilde{\alpha}}P\right|\lesssim\left\langle \xi\right\rangle ^{\left|\alpha\right|-\left|\widetilde{\alpha}\right|}.$
So $P\in S_{1,0}^{\left|\alpha\right|}.$
\item The operator $\widehat{P}=``P\left(x,D\right)''$ is also called the
\textbf{(left) quantization} of $P$.
\item On manifolds, provided that $\frac{1}{2}<\rho\leq1$ and $\rho+\delta\geq1$,
we can define the \textbf{principal symbol} $\sigma_{\mathrm{prin}}\left(\widehat{P}\right)$
in $S_{\rho,\delta}^{m}/S_{\rho,\delta}^{m-\left(\rho-\delta\right)}$
independently of any charts. The principal symbol is a function on
$T^{*}M$. So it is common and convenient to define 
\[
S_{\rho}^{m}=S_{\rho,1-\rho}^{m}\;\;\left(\rho>\frac{1}{2}\right)
\]
\item For convenience, on Riemannian manifolds $\left(M,g\right)$, we use
Pflaum's\textbf{ total symbol}. First we define a cutoff $\chi\in C^{\infty}\left(TM\to[0,1]\right)$
which is $1$ and supported near the zero section $0_{\mathrm{TM}}$
(near enough that the exponential map defines a diffeomorphism from
$W\supset\supp\chi$ onto neighborhood of the diagonal $\Delta\subseteq M\times M$).
We define the \textbf{radius} of $\chi$ as 
\[
\inf\left\{ r>0:\chi\left(x,v\right)=0\;\;\forall\left|v\right|_{g}>r\right\} 
\]
Then for any $u\in C^{\infty}\left(M\right)$ we define the semi-classical
lift $u_{\chi}\in C^{\infty}\left(TM\right)$ 
\[
u_{\chi}\left(x,v\right)=\left\{ \begin{array}{cc}
\chi\left(x,v\right)u\left(\exp_{x}v\right) & \text{ for }\left(x,v\right)\ensuremath{\in}W\\
0 & \text{otherwise}
\end{array}\right.
\]
which is like a ``local trace'' of $u$. Then for any symbol $P\in C^{\infty}\left(T^{*}M\right)$,
we define the operator $\widehat{P}$ by
\begin{equation}
\mathrm{Op}_{\chi}^{\mathrm{Pfl}}\left(u\right)\left(x\right)=\widehat{P}u\left(x\right):=\int_{T_{x}^{*}X}P\left(x,\xi\right)\mathcal{F}\left(u_{\chi}\right)\left(x,\xi\right)\;d\xi\label{eq:total_symbol}
\end{equation}
where the Fourier transform $\mathcal{F}$ is defined by 
\[
\mathcal{F}\left(u_{\chi}\right)\left(x,\xi\right)=\int_{T_{x}X}u_{\chi}\left(x,v\right)e^{-i2\pi\left(\xi\cdot v\right)}\;dv
\]
\item The symbol class $S_{\rho}^{m}\left(M\right)$ (for $m\in\mathbb{R}$
and $\rho>\frac{1}{2}$) consists of $P\in C^{\infty}\left(T^{*}M\right)$
such that for any local trivialization $\left(x,\xi\right):T^{*}M|_{U}\to\mathbb{R}^{2n}$
and compact $K\subseteq U$, we have 
\[
\left|\partial_{\xi}^{\alpha}\partial_{x}^{\beta}P\left(x,\xi\right)\right|\lesssim_{K,\alpha,\beta}\left\langle \xi\right\rangle _{g}^{m-\rho\left|\alpha\right|+\left(1-\rho\right)\left|\beta\right|}\;\forall x\in K,\forall\xi\in T_{x}^{*}M
\]
\end{itemize}
\end{itemize}


\subsubsection{Variable order}
\begin{defn}
An \textbf{order function} $m\left(x,\xi\right)$ is a member of $L^{\infty}\cap S_{r}^{0}$
for $r\in\left(\frac{1}{2},1\right)$. In other words, with any local
trivialization $\left(x,\xi\right):T^{*}M|_{U}\to\mathbb{R}^{2n}$
and any compact $K\subseteq U$
\[
\left|\partial_{\xi}^{\alpha}\partial_{x}^{\beta}m\left(x,\xi\right)\right|\lesssim_{K,\alpha,\beta}\left\langle \xi\right\rangle _{g}^{-r\left|\alpha\right|+\left(1-r\right)\left|\beta\right|}\;\forall x\in K,\forall\xi\in T_{x}^{*}M
\]
and 
\[
\sup_{\left(x,\xi\right)\in T^{*}M}\left|m\left(x,\xi\right)\right|<\infty
\]
We can then define the symbol class $S_{\rho}^{m}=S_{\rho}^{m\left(x,\xi\right)}$.
It consists of $P\in C^{\infty}\left(T^{*}M\right)$ such that with
any local trivialization $\left(x,\xi\right)$ and any compact $K\subseteq U$
as above we get 
\begin{equation}
\left|\partial_{\xi}^{\alpha}\partial_{x}^{\beta}P\left(x,\xi\right)\right|\lesssim_{K,\alpha,\beta}\left\langle \xi\right\rangle _{g}^{m\left(x,\xi\right)-\rho\left|\alpha\right|+\left(1-\rho\right)\left|\beta\right|}\;\forall x\in K,\forall\xi\in T_{x}^{*}M\label{eq:seminorms}
\end{equation}
With $M$ being compact, we can find countably many compact neighborhoods
$K_{j}$ such that $M=\cup_{j\geq1}\mathrm{int}\left(K_{j}\right)$,
and with local trivializations $\left(x,\xi\right)$ near $K_{j}$,
we can define the symbol seminorm
\begin{equation}
\left\Vert P\right\Vert _{m,J}:=\sup_{j\leq J}\sup_{\left|\alpha+\beta\right|\leq J}\;\sup_{x\in K_{j},\xi\in T_{x}^{*}M}\left|\partial_{\xi}^{\alpha}\partial_{x}^{\beta}P\left(x,\xi\right)\right|\left\langle \xi\right\rangle _{g}^{-\left(m\left(x,\xi\right)-\rho\left|\alpha\right|+\left(1-\rho\right)\left|\beta\right|\right)}\label{eq:seminorm_symbol}
\end{equation}
These seminorms induce a Frechet topology on $S_{\rho}^{m}$ (the
topology is unique regardless of the choices of local trivialization). 
\begin{itemize}
\item This implies that locally $\partial_{\xi}^{\alpha}\partial_{x}^{\beta}P\in S^{m-\rho\left|\alpha\right|+\left(1-\rho\right)\left|\beta\right|}$
(note that $m$ is not constant).
\item For any $p\in S_{\rho}^{m},q\in S_{\rho'}^{m'}$ we have $pq\in S_{\min\left(\rho,\rho'\right)}^{m+m'}$. 
\item $S_{\rho}^{m}\subseteq S_{\rho'}^{m'}$ for $m\leq m'$ and $\rho\geq\rho'$.
In particular $S_{\rho}^{m}\subseteq S_{\rho}^{\sup m}$ (traditional
Hormander symbols) and 
\[
S_{\rho}^{m}\subseteq S_{\rho}^{\left(\limsup m\right)+}
\]
Here $\limsup m\left(x,\xi\right)=\sup_{x}\limsup_{\left|\xi\right|_{g}\to\infty}m\left(x,\xi\right)$.
\item Naturally we can use the same residual symbols as Hormander: $S^{-\infty}:=\cap_{m<0}S_{\rho}^{m}$
which is\uline{ independent of \mbox{$\rho$}}, and $S_{\rho}^{\infty}:=\cup_{m>0}S_{\rho}^{m}$.
\item Example: if $m\in L^{\infty}\cap S_{\rho}^{0}$ is an order function
then $\left\langle \xi\right\rangle ^{m\left(x,\xi\right)}\in S_{\rho-}^{m\left(x,\xi\right)}$.
Where the slight loss from $\rho$ to $\rho-$ is due a logarithm
in differentiation. 
\item If $p\in S_{\rho}^{m\left(x,\xi\right)}$ and $\phi:M\to M$ is diffeo
then 
\[
p\circ T^{*}\phi\in S_{\rho}^{m\circ T^{*}\phi}
\]
\item We can then define corresponding \textbf{PDO class} $\Psi_{\rho}^{m\left(x,\xi\right)}$
modulo $\Psi^{-\infty}$ via total symbol as in \eqref{eq:total_symbol}
\[
\forall P\in S_{\rho}^{m}:\widehat{P}u\left(x\right)=\mathrm{Op}_{\chi}^{\mathrm{Pfl}}\left(P\right)u\left(x\right)=\int_{T_{x}^{*}X}p\left(x,\xi\right)\mathcal{F}\left(u_{\chi}\right)\left(x,\xi\right)\;d\xi
\]
In particular $\Psi_{\rho}^{m\left(x,\xi\right)}$ consists of operators
of this form plus smoothing operators. There is not a natural topology
for $\Psi_{\rho}^{m}$. When we need to be explicit about the smoothing
operators, we need to be explicit about the choice of $\chi$.
\item \textbf{Borel summation}: for $\rho<r\leq1$ and $j\in\mathbb{N}_{0}$,
let $p_{j}\in S_{\rho}^{m_{j}\left(x,\xi\right)}$ with variable order
$m_{j}\in S_{r}^{1}$ (\textcolor{red}{why not $S_{r}^{0}$}) such
that $\sup\left|m_{j}\right|\downarrow-\infty$ and $m_{j}\geq m_{j+1}$,
we define $p=\sum_{j\geq0}p_{j}\in S_{\rho}^{m_{0}\left(x,\xi\right)}$
uniquely modulo $S^{-\infty}$ such that
\[
p-\sum_{j=0}^{N-1}p_{j}\in S_{\rho}^{m_{N}}
\]
We also write this as $p\sim\sum_{j=0}^{\infty}p_{j}$.
\begin{itemize}
\item \textbf{Topology}: we define $\ell_{\left(m_{j}\right)}S_{\rho}:=\prod_{j=0}^{\infty}S_{\rho}^{m_{j}\left(x,\xi\right)}$.
With the symbol seminorms from \eqref{eq:seminorm_symbol}, we define
the seminorms
\[
\left\Vert \left(p_{j}\right)_{j=0}^{\infty}\right\Vert _{J}:=\max_{j\leq J}\left\Vert p_{j}\right\Vert _{m_{j},J}\;\forall J\in\mathbb{N}_{0}.
\]
which induce a Frechet topology on $\ell_{\left(m_{j}\right)}S_{\rho}$.
\item \textbf{Continuous Borel summation}: As in \parencite{hintzIntroductionMicrolocalAnalysis2022},
we can choose a continuous nonlinear map $\Sigma_{\mathcal{A}}:\ell_{\left(m_{j}\right)}S_{\rho}\to S_{\rho}^{m_{0}\left(x,\xi\right)}$
such that $\Sigma_{\mathcal{A}}\left(p_{j}\right)_{j=0}^{\infty}\sim\sum_{j=0}^{\infty}p_{j}$.
\end{itemize}
\item With $p\in S_{\rho}^{m\left(x,\xi\right)}$ we define the \textbf{principal
symbol} as $\sigma_{\mathrm{prin}}\left(\widehat{p}\right)=\left[p\right]\in S_{\rho}^{m\left(x,\xi\right)}/S_{\rho}^{m\left(x,\xi\right)-\left(2\rho-1\right)}$.
\item Adjoint: with $p\in S_{\rho}^{m\left(x,\xi\right)}$ and $\hat{p}\in\Psi_{\rho}^{m\left(x,\xi\right)}$
we can define formal $L^{2}$-adjoint $\hat{p}^{*}\in\Psi_{\rho}^{m\left(x,\xi\right)}$
with symbol $p^{*}\in S_{\rho}^{m\left(x,\xi\right)}$ such that 
\[
\sigma_{\mathrm{prin}}\left(\hat{p}^{*}\right)=\overline{p}
\]
\item \textbf{Composition}: with $p\in S_{\rho}^{m\left(x,\xi\right)},q\in S_{\rho}^{m'\left(x,\xi\right)}$
(same $\rho$), we have $\hat{p}\hat{q}\in\Psi_{\rho}^{m\left(x,\xi\right)+m'\left(x,\xi\right)}$
and
\[
\sigma_{\mathrm{prin}}\left(\widehat{p}\widehat{q}\right)=\sigma_{\mathrm{prin}}\left(\hat{p}\right)\sigma_{\mathrm{prin}}\left(\hat{q}\right)
\]

\begin{itemize}
\item Previously we also showed $pq\in S_{\rho}^{m+m'}$.
\item \textbf{Topology}: recall that $S_{\rho}^{m}$ is a Frechet space
(from countable seminorms from \eqref{eq:seminorms}. On the other
hand, each $R\in\Psi^{-\infty}$ with smooth Schwartz kernel $K_{R}\left(x,y\right)$
can inherit the Frechet topology from the $C^{\infty}$ seminorms
on $K_{R}$. 
\item \textbf{Continuity of composition}: for a fixed cutoff $\chi$ with
small enough radius, and $a\in S_{\rho}^{m},b\in S_{\rho}^{m'}$,
we can choose local continuous nonlinear maps $\left(a,b\right)\mapsto a\#_{\chi}b\in S_{\rho}^{m+m'}$
and $\left(a,b\right)\mapsto R_{\chi}\left(a,b\right)\in\Psi^{-\infty}$
such that 
\begin{equation}
\mathrm{Op}_{\chi}^{\mathrm{Pfl}}\left(a\right)\circ\mathrm{Op}_{\chi}^{\mathrm{Pfl}}\left(b\right)=\mathrm{Op}_{\chi}^{\mathrm{Pfl}}\left(a\#_{\chi}b\right)+R_{\chi}\left(a,b\right)\label{eq:composition}
\end{equation}
Here, ``local'' means on a neighborhood surrounding any given point.
This boils down to picking partitions of unity and coordinate patches,
along with continuous choices of Borel summations.
\end{itemize}
\item \textbf{Egorov} (special case): let $\hat{p}\in\Psi_{\rho}^{m\left(x,\xi\right)}$
with symbol $p\in S_{\rho}^{m\left(x,\xi\right)}$ and $f:M\to M$
diffeomorphism. Previously we showed $p\circ T^{*}\left(f^{-1}\right)\in S_{\rho}^{m\circ T^{*}\left(f^{-1}\right)}$.
With $\hat{F}:u\mapsto u\circ f$ we have 
\[
\hat{F}^{-1}\hat{p}\widehat{F}\in\Psi_{\rho}^{m\circ T^{*}\left(f^{-1}\right)}
\]
and $\sigma_{\mathrm{prin}}\left(\hat{F}^{-1}\hat{p}\widehat{F}\right)=p\circ T^{*}\left(f^{-1}\right)\text{ modulo }S_{\rho}^{m\circ T^{*}\left(f^{-1}\right)-\left(2\rho-1\right)}$.
\begin{itemize}
\item In particular $\hat{F}^{-1}\hat{p}\widehat{F}\left(\phi\right)=\hat{F}^{-1}\hat{p}\left(\phi\circ f\right)=\left(\hat{p}\left(\phi\circ f\right)\right)\circ f^{-1}$.
Conjugation by $f$ basically changes the principal symbol in the
obvious way, by the corresponding lift $T^{*}\left(f^{-1}\right)$.
\item The proof relies on choosing a cutoff for Schwartz kernel near the
diagonal, so that the diffeomorphism $f$ can be approximated (after
local trivialization) by 
\[
f\left(x\right)-f\left(y\right)=\left(\int_{0}^{1}\left(x-y\right)\cdot\nabla f\left(y+t\left(x-y\right)\right)\;dt\right)=\Phi\left(x,y\right)\left(x-y\right)
\]
where $\Phi\left(x,y\right)$ is invertible and $\Phi\left(x,x\right)=f'\left(x\right)=Df\left(x\right).$
In particular we have $e^{i2\pi\left(f\left(x\right)-f\left(y\right)\right)\cdot\xi}=e^{i2\pi\left(x-y\right)\cdot\Phi\left(x,y\right)^{T}\xi}$.
\item \textbf{Topology}: let $\left(f_{a}\right)$ be a family of diffeomorphisms
on $M$. We say $f_{a}\to f$ when for any $\phi\in C^{\infty}\left(M\right):$
\[
\phi\circ f_{a}\xrightarrow{C^{\infty}}\phi\circ f.
\]
\item \textbf{Continuous Egorov}: with a fixed cutoff $\chi$ with small
enough radius, for any $p\in S_{\rho}^{m\left(x,\xi\right)}$ and
$f:M\to M$ diffeomorphism, we can choose local continuous nonlinear
maps $\left(p,f\right)\mapsto E_{\chi}\left(p,f\right)\in S_{\rho}^{m\circ T^{*}\left(f^{-1}\right)-\left(2\rho-1\right)}$
and $\left(p,f\right)\mapsto R_{\chi,p,f}\in\Psi^{-\infty}$such that
\begin{equation}
\left(f^{*}\right)^{-1}\circ\mathrm{Op}_{\chi}^{\mathrm{Pfl}}\left(p\right)\circ f^{*}=\mathrm{Op}_{\chi}^{\mathrm{Pfl}}\left(p\circ T^{*}\left(f^{-1}\right)\right)+\mathrm{Op}_{\chi}^{\mathrm{Pfl}}E_{\chi}\left(p,f\right)+R_{\chi,p,f}\label{eq:continuous_egorov}
\end{equation}
\end{itemize}
\item \textbf{Sobolev continuity}: $\hat{p}\in\Psi_{\rho}^{m\left(x,\xi\right)}$
is a continuous map $H^{s}\to H^{s-\limsup m}$.
\item \textbf{(Variable-order) Ellipticity}: $p\in S_{\rho}^{m\left(x,\xi\right)}$
is \textbf{elliptic symbol} if
\[
\left|p\left(x,\xi\right)\right|\gtrsim\left\langle \xi\right\rangle ^{m\left(x,\xi\right)}\text{ for }\left\langle \xi\right\rangle \gtrsim1
\]
Equivalently, there is $q\in S_{\rho}^{-m(x,\xi)}$ such that $pq-1\in S_{\rho}^{-\infty}$.
Equivalently $\hat{p}$ has a \textbf{parametrix}, i.e. there is $\hat{q}\in\Psi_{\rho}^{-m\left(x,\xi\right)}$
such that $\hat{p}\hat{q}-1$ and $\hat{q}\hat{p}-1\in\Psi^{-\infty}$.
\begin{itemize}
\item If $p\in S_{\rho}^{m\left(x,\xi\right)}$ is elliptic symbol and $q\in S_{\rho}^{m\left(x,\xi\right)}$
such that 
\[
p-q\in S_{\rho}^{m\left(x,\xi\right)-\epsilon}\text{ for some }\epsilon>0
\]
then $q$ is also elliptic. In other words, only top power matters.
\item Note that this notion of ellipticity is more general than usual, since
$m\left(x,\xi\right)$ could have negative values.
\item An operator is called elliptic if it has an \textbf{elliptic symbol}. 
\item \textbf{Hormander's square root trick}: assume $\hat{p}\in\Psi_{\rho}^{m\left(x,\xi\right)}$
is formally self-adjoint and elliptic. Assume there is $q\in S_{\rho}^{m}$
real-valued such that $q-p\in S_{\rho}^{m-\left(2\rho-1\right)}$
and
\[
\min_{x}\limsup_{\left|\xi\right|_{g}\to\infty}q\left(x,\xi\right)>0
\]
then there is $\hat{b}\in\Psi_{\rho}^{\frac{1}{2}m\left(x,\xi\right)}$
such that 
\[
\hat{p}-\hat{b}^{*}\hat{b}\in\Psi^{-\infty}
\]

\begin{itemize}
\item \textbf{Continuity of square root}: because the square root is defined
by Borel summation, with a fixed cutoff $\chi$ with small enough
radius, with $p$ and $q$ as above, we can choose local continuous
nonlinear maps $\left(p,q\right)\mapsto\mathrm{SR}_{\chi}\left(p,q\right)\in S_{\rho}^{\frac{1}{2}m\left(x,\xi\right)}$
such that 
\begin{equation}
\left(p,q\right)\mapsto\mathrm{Op}_{\chi}^{\mathrm{Pfl}}\left(p\right)-\mathrm{Op}_{\chi}^{\mathrm{Pfl}}\left(\mathrm{SR}_{\chi}\left(p,q\right)\right)^{*}\mathrm{Op}_{\chi}^{\mathrm{Pfl}}\left(\mathrm{SR}_{\chi}\left(p,q\right)\right)\in\Psi^{-\infty}\label{eq:square_root_cont}
\end{equation}
is also continuous.
\item \textcolor{red}{Faure only assumes $p-\mathrm{Re}\left(p\right)\in S_{\rho}^{m\left(x,\xi\right)-\epsilon}$
for some $\epsilon>0$ (so $p$ might not be real and $\hat{p}$ might
not be self-adjoint). This might be an error from Faure, since Borel
summation wouldn't work without real principal symbols at each stage.} 
\end{itemize}
\item \textbf{Half-fredholm}: if $\hat{p}\in\Psi_{\rho}^{m\left(x,\xi\right)}$
is elliptic then the kernel of $\widehat{p}:H^{s}\to H^{s-\limsup m}$
is finite-dimensional and contained in $C^{\infty}\left(M\right)$.
Furthermore, if $\hat{p}$ is formally self-adjoint then $\hat{p}$
as unbounded operator on $L^{2}$ has a \uline{self-adjoint extension}
(Friedrichs extension via square roots), and there is $\hat{r}\in\Psi_{\rho}^{-\infty}$
such that $\hat{p}+\hat{r}:C^{\infty}\to C^{\infty}$ has an actual
inverse in $\Psi_{\rho}^{-m\left(x,\xi\right)}$.
\begin{itemize}
\item As a consequence, if $p\in S_{\rho}^{m\left(x,\xi\right)}$ is real-valued
$\left(\overline{p}=p\right)$ elliptic symbol, then $p=p^{*}$ modulo
$S_{\rho}^{m\left(x,\xi\right)-\left(2\rho-1\right)}$ and there is
a modification $q$ such that $\hat{q}=\frac{1}{2}\left(\widehat{p}+\widehat{p}^{*}\right)\text{ modulo }S^{-\infty},\sigma_{\mathrm{prin}}\left(\hat{p}\right)=\sigma_{\mathrm{prin}}\left(\hat{q}\right)$
and $q$ is formally self-adjoint + invertible.
\item Standard constant-order elliptic PDOs (like the Laplacian) are actually
Fredholm (finite-dim ker and coker)
\end{itemize}
\end{itemize}
\item \textbf{Quasi-compactness}: let $p\in S_{\rho}^{0}$ and $L:=\limsup\left|p\right|$.
Then for any $\epsilon>0$ 
\begin{align*}
\hat{q} & :=\left(L^{2}+\epsilon\right)-\hat{p}^{*}\hat{p}\in\Psi_{\rho}^{0}\text{ is self-adjoint}\\
q & =\left(L^{2}+\epsilon\right)-\left|p\right|^{2}\text{ modulo }S_{\rho}^{-\left(2\rho-1\right)}
\end{align*}
Taking square root we get $\hat{q}=\hat{b}^{*}\hat{b}-\hat{K}$ where
$\hat{K}\in S^{-\infty}$. This leads to
\begin{align*}
\left\Vert \hat{p}\phi\right\Vert _{L^{2}}^{2} & =\left\langle \hat{p}^{*}\hat{p}\phi,\phi\right\rangle =\left(L^{2}+\epsilon\right)\left\Vert \phi\right\Vert _{L^{2}}^{2}-\left\langle \hat{q}\phi,\phi\right\rangle \\
 & =\left(L^{2}+\epsilon\right)\left\Vert \phi\right\Vert _{L^{2}}^{2}-\left\Vert \hat{b}\phi\right\Vert _{L^{2}}^{2}+\left\langle \hat{K}\phi,\phi\right\rangle \\
 & \leq\left(L^{2}+\epsilon\right)\left\Vert \phi\right\Vert _{L^{2}}^{2}+\left\langle \hat{K}\phi,\phi\right\rangle 
\end{align*}
On the torus it is Lasota-Yorke if we let $L^{2}+\epsilon<1$.\\
By spectral projection of the Laplacian (a replacement for Littlewood-Paley),
there is a decomposition
\begin{equation}
\hat{p}=\hat{p}_{\epsilon}+\hat{K}_{\epsilon}\label{eq:decomposition_quasi}
\end{equation}
where $\widehat{K}_{\epsilon}\in\Psi^{-\infty}$ and $\left\Vert \hat{p}_{\epsilon}\right\Vert _{L^{2}\to L^{2}}\leq L+\epsilon$. 
\end{itemize}
\end{defn}


\subsection{Anisotropic Sobolev}

Assume $M,f,\hat{F}$ as in Subsection \prettyref{subsec:Setting}. 

Let $u<0<s$. We define the order function $m\left(x,\xi\right)\in S_{1}^{0}$
such that
\begin{enumerate}
\item $u\leq m\left(x,\xi\right)\leq s$
\item $m\left(x,\xi\right)=m\left(x,\frac{\xi}{\left|\xi\right|}\right)\;\forall x,\forall\left|\xi\right|>1$
\item $m\left(x,\xi\right)=s$ for $\xi$ near $E_{s}^{*}\left(x\right)$,
and $m\left(x,\xi\right)=u$ for $\xi$ near $E_{u}^{*}\left(x\right)$.
Note that $E_{s}^{*},E_{u}^{*}$ depend on $f$.
\item $m$ decreases along $T^{*}\left(f^{-1}\right)$
\[
m\circ T^{*}\left(f^{-1}\right)\left(x,\xi\right)\leq m\left(x,\xi\right)\text{ for }\left|\xi\right|\gtrsim1
\]
\end{enumerate}
We define the \textbf{escape function}
\begin{equation}
A_{m}\left(x,\xi\right):=\left\langle \xi\right\rangle ^{m\left(x,\xi\right)}\in S_{1-}^{m\left(x,\xi\right)}\label{eq:A_m}
\end{equation}
Then 
\begin{equation}
A_{m}\circ T^{*}\left(f^{-1}\right)\left(x,\xi\right)\leq e^{-c_{2}\min\left(-u,s\right)}A_{m}\left(x,\xi\right)\text{ for }\left|\xi\right|\gtrsim1\label{eq:c_2_escape}
\end{equation}
where $c_{2}$ is independent of the choice of $u,s$. Here $c_{2}$
can be arbitrarily close to $\left|\ln\left(c^{2}\theta\right)\right|$
from \eqref{eq:smoothened-1}.
\begin{itemize}
\item The foliations $E_{s}^{*}\left(x\right)$ and $E_{u}^{*}\left(x\right)$
only have Holder regularity, but $m$ is still smooth.
\item As $A_{m}$ is real + variable-order elliptic, picking \uline{\mbox{$\rho$}
arbitrarily close to \mbox{$1$}}, we can modify $A_{m}$ into $A_{m}'$
such that 
\begin{enumerate}
\item $A_{m}'=A_{m}$ modulo $S_{\rho}^{m\left(x,\xi\right)-(2\rho-1)}$.
\item $\widehat{A_{m}'}=\frac{1}{2}\left(\widehat{A_{m}}+\widehat{A_{m}}^{*}\right)\text{ modulo }S^{-\infty}$
\item $\widehat{A_{m}'}$ is formally self-adjoint on $L^{2}$ and invertible
on $C^{\infty}\left(M\right)$ with inverse $\widehat{A_{m}'}^{-1}\in S_{\rho}^{-m}$.
\end{enumerate}
\end{itemize}
\begin{claim}
For any $\phi\in C^{\infty}:$
\begin{equation}
\left\Vert \widehat{A_{m}'}\phi\right\Vert _{L^{2}}\sim\left\Vert \widehat{A_{m}}\phi\right\Vert _{L^{2}}+\left\Vert \phi\right\Vert _{H^{-\max\left|m\right|}}\label{eq:modificaiton}
\end{equation}
\end{claim}

\begin{proof}
We first observe that $\forall\phi\in C^{\infty}:\left\Vert \left(\widehat{A_{m}}-\widehat{A_{m}'}\right)\widehat{A_{m}'}^{-1}\phi\right\Vert _{L^{2}}\lesssim\left\Vert \phi\right\Vert _{L^{2}}$
as $\left(\widehat{A_{m}}-\widehat{A_{m}'}\right)\widehat{A_{m}'}^{-1}\in S_{\rho}^{-\left(2\rho-1\right)}$.
So $\left\Vert \left(\widehat{A_{m}}-\widehat{A_{m}'}\right)\phi\right\Vert _{L^{2}}\lesssim\left\Vert \widehat{A_{m}'}\phi\right\Vert _{L^{2}}$
and $\left\Vert \widehat{A_{m}}\phi\right\Vert _{L^{2}}\lesssim\left\Vert \widehat{A_{m}'}\phi\right\Vert _{L^{2}}$.

Since $\widehat{A_{m}'}^{-1}$ maps $L^{2}\to H^{-\max\left|m\right|}$
continuously, we have 
\[
\left\Vert \widehat{A_{m}}\phi\right\Vert _{L^{2}}+\left\Vert \phi\right\Vert _{H^{-\max\left|m\right|}}\lesssim\left\Vert \widehat{A_{m}'}\phi\right\Vert _{L^{2}}.
\]
For the other direction, let $\widehat{Q_{m}}\in\Psi_{\rho}^{-m}$
be a parametrix of $\widehat{A_{m}}$, and we have 
\[
\left\Vert \left(\widehat{A_{m}}-\widehat{A_{m}'}\right)\widehat{Q_{m}}\phi\right\Vert _{L^{2}}\lesssim\left\Vert \phi\right\Vert _{L^{2}}\;\forall\phi\in C^{\infty}
\]
Which then implies $\left\Vert \left(\widehat{A_{m}}-\widehat{A_{m}'}\right)\widehat{Q_{m}}\widehat{A_{m}}\phi\right\Vert _{L^{2}}\lesssim\left\Vert \widehat{A_{m}}\phi\right\Vert _{L^{2}}$.
As $\widehat{Q_{m}}\widehat{A_{m}}-1\in S^{-\infty}$: 
\[
\left\Vert \widehat{A_{m}'}\phi\right\Vert _{L^{2}}\leq\left\Vert \widehat{A_{m}}\phi\right\Vert _{L^{2}}+\left\Vert \left(\widehat{A_{m}}-\widehat{A_{m}'}\right)\phi\right\Vert _{L^{2}}\lesssim\left\Vert \widehat{A_{m}}\phi\right\Vert _{L^{2}}+\left\Vert \phi\right\Vert _{H^{-\max\left|m\right|}}
\]
 We are done.
\end{proof}
We then define the anisotropic Sobolev space 
\begin{align}
H^{m} & =\widehat{A_{m}'}^{-1}\left(L^{2}\left(M\right)\right)\label{eq:aniso_sobolev}\\
\left\Vert \phi\right\Vert _{H^{m}} & =\left\Vert \widehat{A_{m}'}\phi\right\Vert _{L^{2}}
\end{align}
Note that $m$ is not constant. This is similar to $H^{s}\left(\mathbb{R}^{d}\right)=\widehat{\left\langle \xi\right\rangle ^{s}}^{-1}\left(L^{2}\left(\mathbb{R}^{d}\right)\right)\;\forall s\in\mathbb{R}$.
In particular $H^{m}$ is a Hilbert space with product 
\[
\left\langle \phi,\psi\right\rangle _{H^{m}}=\left\langle \widehat{A_{m}'}\phi,\widehat{A_{m}'}\psi\right\rangle _{L^{2}}
\]
where we use the self-adjointness of $\widehat{A_{m}'}$. Then $\widehat{A_{m}'}:H^{m}\to L^{2}$
is a unitary map. Obviously 
\[
H^{\max m}\subseteq H^{m}\subseteq H^{\min m}
\]
and $H^{m}\hookrightarrow H^{m'}$is dense embedding for any $m\geq m'$.
Also trivially, smooth multipliers are continuous on $H^{m}$. 

The dual of $H^{m}$ is 
\[
H^{-m}=\widehat{A_{m}'}\left(L^{2}\left(M\right)\right)=\left(H^{m}\right)^{*}
\]

We now discuss the transfer operator $\widehat{F}$. 
\begin{itemize}
\item The $L^{2}$-adjoint $\widehat{F}^{*}$is 
\[
\widehat{F}^{*}\phi\left(y\right)=\frac{\phi\left(f^{-1}y\right)}{\left|\det D_{f^{-1}y}f\right|}
\]
\item $\widehat{F}$ maps from $H^{m}$ to $H^{m}$ continuously by Egorov.
Equivalently, we have
\begin{align*}
\left\Vert \widehat{F}^{-1}\widehat{A_{m}'}\hat{F}\widehat{A_{m}'}^{-1}\phi\right\Vert _{L^{2}} & \lesssim\left\Vert \phi\right\Vert _{L^{2}}
\end{align*}
Which is true because $\widehat{F}^{-1}\widehat{A_{m}'}\hat{F}$ is
PDO by Egorov, and 
\[
\sigma_{\mathrm{prin}}\left(\widehat{F}^{-1}\widehat{A_{m}'}\hat{F}\widehat{A_{m}'}^{-1}\right)=\sigma_{\mathrm{prin}}\left(\widehat{F}^{-1}\widehat{A_{m}'}\hat{F}\right)\sigma_{\mathrm{prin}}\left(\widehat{A_{m}'}^{-1}\right)=\frac{A_{m}\circ T^{*}\left(f^{-1}\right)}{A_{m}}
\]
And we have $\limsup\frac{A_{m}\circ T^{*}\left(f^{-1}\right)}{A_{m}}\leq e^{-c_{2}\min\left(-u,s\right)}$
by \eqref{eq:c_2_escape}. So by the quasi-compactness decomposition
in \eqref{eq:decomposition_quasi}, we obtain
\begin{equation}
\widehat{F}=\widehat{r}_{m}+\widehat{k}_{m}\label{eq:decompo}
\end{equation}
where $\widehat{k}_{m}$ is a compact operator (from $\Psi^{-\infty}$
operators) and 
\[
\left\Vert \widehat{r}_{m}\right\Vert _{L^{2}\to L^{2}}\leq\left\Vert \widehat{F}\right\Vert _{L^{2}\to L^{2}}e^{-c_{2}\min\left(-u,s\right)}
\]
where $c_{2}$ is from \eqref{eq:c_2_escape}. Consequently the essential
spectral radius of $\widehat{F}$ is smaller than $\left\Vert \widehat{F}\right\Vert _{L^{2}\to L^{2}}e^{-c_{2}\min\left(-u,s\right)}$.
The discrete spectrum of $\hat{F}$ (\textbf{Ruelle resonances}) is
outside that ball, independent of the choice of $m$, and there is
a general Jordan decomposition for $\widehat{k}_{m}$. There are also
implications for meromorphic extension of resolvent $\left(z-\widehat{F}\right)^{-1}$.
\end{itemize}

\subsection{Application to the CAT map problem}

\subsubsection{Equivalence between Faure's norm and the CAT norm}

For the cat map problem in this paper, we specialize the escape function
$A_{m}$ from \eqref{eq:A_m} to 
\[
A_{m}\left(x,\xi\right):=\left\langle \xi\right\rangle ^{m\left(\xi\right)}=\left\langle \xi\right\rangle ^{p\alpha\left(\xi\right)}\in S_{1-}^{m\left(x,\xi\right)}\subseteq S_{1-}^{\max m}\left(\mathbb{T}^{2}\right)
\]
We then define $\widehat{A_{m}'}$ as in \eqref{eq:modificaiton}.
Then we have 
\[
\left\Vert \widehat{A_{m}'}\phi\right\Vert _{L^{2}}\sim\left\Vert \widehat{A_{m}}\phi\right\Vert _{L^{2}}+\left\Vert \phi\right\Vert _{H^{-\max\left|m\right|}}
\]
We note that $\widehat{A_{m}}\phi$ is defined by Pflaum total symbol
from \eqref{eq:total_symbol}, which requires a cutoff $\chi$. We
now specify the cutoff $\chi\left(x,y\right)=\chi\left(y\right)$
such that $\chi\left(y\right)=0$ whenever $\left|y\right|>\frac{1}{4}$.

We now find the Ruhanzsky-Turunen toroidal symbol of $\widehat{A_{m}}$
\parencite{ruzhanskyQuantizationPseudodifferentialOperators2010}
by the computation 
\begin{align}
\forall\left(x,k\right)\in\mathbb{T}^{2}\times\mathbb{R}^{2}:\sigma_{\mathbb{T}^{2}}\left(\widehat{A_{m}}\right)\left(x,k\right) & :=e_{-k}\left(x\right)\left(\widehat{A_{m}}e_{k}\right)\left(x\right)\nonumber \\
 & =e_{-k}\left(x\right)\int_{B\left(0,\frac{1}{4}\right)}dh\int_{\mathbb{R}^{2}}d\xi\;\left\langle \xi\right\rangle ^{m\left(\xi\right)}e_{k}\left(x+h\right)\chi\left(h\right)e_{-\xi}\left(h\right)\nonumber \\
 & =\int_{\mathbb{R}^{2}}d\xi\;\left\langle \xi\right\rangle ^{m\left(\xi\right)}\underbrace{\int_{B\left(0,\frac{1}{4}\right)}dh\;e_{k-\xi}\left(h\right)\chi\left(h\right)}_{\mathcal{F}\chi\left(\xi-k\right)}\\
 & =\int_{\mathbb{R}^{2}}d\xi\;\left\langle \xi\right\rangle ^{m\left(\xi\right)}\mathcal{F}\chi\left(\xi-k\right)=\int_{\mathbb{R}^{2}}d\xi\;\left\langle \xi+k\right\rangle ^{m\left(\xi+k\right)}\mathcal{F}\chi\left(\xi\right)
\end{align}
Here we note that $\mathcal{F}\chi$ is Schwartz with $\mathcal{F}\chi\left(0\right)=\int\chi>0$,
while $\int\mathcal{F}\chi=\chi\left(0\right)=1$. 
\begin{claim}
For large $\left|k\right|$ we have $\left|\sigma_{\mathbb{T}^{2}}\left(\widehat{A_{m}}\right)\left(x,k\right)\right|\sim\left\langle k\right\rangle ^{m\left(k\right)}$
\end{claim}

\begin{proof}
We make the important cutoff at $\left|\xi\right|=\left|k\right|^{\frac{1}{2}}$.
Letting $\left|k\right|\to\infty$ we have 
\begin{equation}
\int_{\left|\xi\right|<\left|k\right|^{\frac{1}{2}}}\mathcal{F}\chi\left(\xi\right)\;d\xi=1+o_{k}\left(1\right)\label{eq:nearly1}
\end{equation}
For $M=5\max\left|m\right|+10$ we have
\begin{align*}
\int_{\left|\xi\right|>\left|k\right|^{\frac{1}{2}}}\frac{\left\langle k+\xi\right\rangle ^{m\left(k+\xi\right)}}{\left\langle k\right\rangle ^{m\left(k\right)}}\left|\mathcal{F}\chi\left(\xi\right)\right|\;d\xi\; & \lesssim\int_{\left|\xi\right|>\left|k\right|^{\frac{1}{2}}}\left(\left|k\right|^{2\max\left|m\right|}+\left|\xi\right|^{2\max\left|m\right|}\right)\frac{o_{k}\left(1\right)}{\left|\xi\right|^{M}}\;d\xi\\
 & \lesssim\int_{\left|\zeta\right|>1}\left(\left|k\right|^{2\max\left|m\right|}+\left(\left|\zeta\right|^{2}\left|k\right|\right)^{\max\left|m\right|}\right)\left|k\right|^{-\frac{M}{2}+\frac{2}{2}}\frac{o_{k}\left(1\right)}{\left|\zeta\right|^{M}}\;d\zeta\\
 & =o_{k}\left(1\right)
\end{align*}
The crucial observation is that for large $\left|k\right|$ 
\[
\frac{\left\langle k+\xi\right\rangle ^{m\left(k+\xi\right)}}{\left\langle k\right\rangle ^{m\left(k\right)}}=1+o_{k}\left(1\right)\;\forall\xi\in B\left(k,\left|k\right|^{\frac{1}{2}}\right)
\]
which, along with \eqref{eq:nearly1}, implies
\begin{align*}
 & \int_{\left|\xi\right|<\left|k\right|^{\frac{1}{2}}}\frac{\left\langle k+\xi\right\rangle ^{m\left(k+\xi\right)}}{\left\langle k\right\rangle ^{m\left(k\right)}}\mathcal{F}\chi\left(\xi\right)\;d\xi\\
 & =\int_{\left|\xi\right|<\left|k\right|^{\frac{1}{2}}}\left(1+o_{k}\left(1\right)\right)\mathcal{F}\chi\left(\xi\right)\;d\xi\\
 & =\int_{\left|\xi\right|<\left|k\right|^{\frac{1}{2}}}\mathcal{F}\chi\left(\xi\right)\;d\xi+O\left(o_{k}\left(1\right)\int_{\mathbb{R}^{2}}\left|\mathcal{F}\chi\left(\xi\right)\right|\;d\xi\right)=1+o_{k}\left(1\right)
\end{align*}
And we are done.
\end{proof}
Let $a_{m}=\sigma_{\mathbb{T}^{2}}\left(\widehat{A_{m}}\right)$.
The explicit calculation above also guarantees $a_{m}\in S_{1-}^{\max m}\left(\mathbb{T}^{n}\times\mathbb{Z}^{n}\right)$
as defined by Ruhanzsky-Turunen. 

Another crucial observation is that $a_{m}$ does not depend on $x$,
so $a_{m}\left(x,k\right)=a_{m}\left(k\right)$. We need this to preserve
orthogonality in $L^{2}$-based norms. 

It is easy to check via toroidal quantization that $\widehat{a_{m}}=\widehat{A_{m}}$,
i.e. $\forall\phi\in C^{\infty}\left(\mathbb{T}^{2}\right)$
\begin{align*}
\widehat{a_{m}}\phi\left(x\right) & :=\sum_{k\in\mathbb{Z}^{2}}a_{m}\left(k\right)\mathcal{F}_{\mathbb{T}^{2}}\phi\left(k\right)e_{k}\left(x\right)=\sum_{k\in\mathbb{Z}^{2}}\sigma_{\mathbb{T}^{2}}\left(\widehat{A_{m}}\right)\left(x,k\right)\mathcal{F}_{\mathbb{T}^{2}}\phi\left(k\right)e_{k}\left(x\right)\\
 & =\sum_{k\in\mathbb{Z}^{2}}\left(\widehat{A_{m}}e_{k}\right)\left(x\right)\mathcal{F}_{\mathbb{T}^{2}}\phi\left(k\right)=\widehat{A_{m}}\left(\sum_{k\in\mathbb{Z}^{2}}\mathcal{F}_{\mathbb{T}^{2}}\phi\left(k\right)e_{k}\right)\left(x\right)=\widehat{A_{m}}\phi\left(x\right)
\end{align*}
We then obtain the fact that 
\begin{align*}
\left\Vert \widehat{A_{m}}\phi\right\Vert _{L^{2}}^{2} & =\left\Vert \widehat{a_{m}}\phi\right\Vert _{L^{2}}^{2}=\left|\mathcal{F}_{\mathbb{T}^{2}}\phi\left(0\right)\right|^{2}+\sum_{k\in\mathbb{Z}^{2}\backslash\left\{ 0\right\} }\left|a_{m}\left(k\right)\right|^{2}\left|\mathcal{F}_{\mathbb{T}^{2}}\phi\left(k\right)\right|^{2}\\
 & \lesssim\left\Vert P_{\lesssim1}\phi\right\Vert _{L^{2}}^{2}+\sum_{\left|k\right|\gtrsim1}\left\langle k\right\rangle ^{2m\left(k\right)}\left|\mathcal{F}_{\mathbb{T}^{2}}\phi\left(k\right)\right|^{2}\sim\left\Vert \phi\right\Vert _{\mathrm{CAT}}^{2}
\end{align*}
and 
\begin{align*}
\left\Vert \phi\right\Vert _{\mathrm{CAT}}^{2} & \lesssim\left\Vert P_{\lesssim1}\phi\right\Vert _{L^{2}}^{2}+\left\Vert P_{\gtrsim1}\phi\right\Vert _{L^{2}}^{2}\lesssim\left\Vert \phi\right\Vert _{H^{-\max\left|m\right|}}^{2}+\sum_{\left|k\right|\gtrsim1}\left|a_{m}\left(k\right)\right|^{2}\left|\mathcal{F}_{\mathbb{T}^{2}}\phi\left(k\right)\right|^{2}\\
 & \lesssim\left\Vert \widehat{A_{m}}\phi\right\Vert _{L^{2}}^{2}+\left\Vert \phi\right\Vert _{H^{-\max\left|m\right|}}^{2}
\end{align*}
And therefore 
\[
\left\Vert \widehat{A_{m}'}\phi\right\Vert _{L^{2}}^{2}\sim\left\Vert \widehat{A_{m}}\phi\right\Vert _{L^{2}}^{2}+\left\Vert \phi\right\Vert _{H^{-p}}^{2}\sim\left\Vert \phi\right\Vert _{\mathrm{CAT}}^{2}+\left\Vert \phi\right\Vert _{H^{-p}}^{2}\sim\left\Vert \phi\right\Vert _{\mathrm{CAT}}^{2}.
\]


\subsubsection{Uniform Lasota-Yorke}

The uniform Lasota-Yorke estimate is a simple consequence of the following
decomposition.
\begin{claim}
There is a decomposition
\[
\mathcal{L}_{f_{a}}=\widehat{r_{a}}+\widehat{k_{a}}
\]
 where $\left\Vert \widehat{r_{a}}\right\Vert _{H^{m}\to H^{m}}\leq e^{-c_{3}p}$
for some $c_{3}>0$ independent of small $a$, and $\widehat{k_{a}}$
is a smoothing operator with norms uniform in $a$. In other words
\begin{equation}
\forall s_{1},s_{2}\in\mathbb{R}:\left\Vert \widehat{k_{a}}\right\Vert _{H^{s_{1}}\to H^{s_{2}}}\lesssim_{s_{1},s_{2},\neg a}1\label{eq:uniform_smoothing}
\end{equation}
\end{claim}

\begin{proof}
We fix $\rho<1$ as an unimportant constant arbitrarily close to $1$.
Also recall that PDOs are defined by Pflaum's total symbol, which
requires a cutoff $\chi$. We fix a cutoff $\chi$ such that $\chi\left(x,v\right)=\chi\left(v\right)=0\;\;\forall\left|v\right|>\frac{1}{100}$.

Let $a\to0$. Recall that $C^{\infty}\left(\mathbb{T}^{2}\right)$
is a Frechet space and $\forall\phi\in C^{\infty}\left(\mathbb{T}^{2}\right):$
\[
\phi\circ f_{a}\xrightarrow[a\to0]{C^{\infty}}\phi\circ f,\text{ and }\phi\circ f_{a}^{-1}\xrightarrow[a\to0]{C^{\infty}}\phi\circ f^{-1}
\]
By Egorov, we know $\mathcal{L}_{f_{a}}^{-1}\widehat{A_{m}'}\mathcal{L}_{f_{a}}\in\Psi_{\rho}^{m\circ T^{*}f_{a}}$.
Since $m\circ T^{*}f_{a}\leq m$ for small $a$, we define $\tilde{m}=\sup_{a\in\left(0,\tilde{a}\right)}m\circ T^{*}f_{a}$.
Then we still have $\tilde{m}\leq m$ for small $\tilde{a}$, and
with the notation from \eqref{eq:continuous_egorov}, we have 
\begin{align*}
\mathcal{L}_{f_{a}}^{-1}\widehat{A_{m}'}\mathcal{L}_{f_{a}} & =\left(\mathcal{L}_{f_{a}}\right)^{-1}\mathrm{Op}_{\chi}^{\mathrm{Pfl}}\left(A_{m}'\right)\mathcal{L}_{f_{a}}=\mathrm{Op}_{\chi}^{\mathrm{Pfl}}\left(A_{m}'\circ T^{*}f_{a}\right)+\mathrm{Op}_{\chi}^{\mathrm{Pfl}}E_{\chi}\left(A_{m}',f_{a}^{-1}\right)+R_{\chi,A_{m}',f_{a}^{-1}}\in\Psi_{\rho}^{\widetilde{m}}
\end{align*}
where $A_{m}'\circ T^{*}f_{a}$, $E_{\chi}\left(A_{m}',f_{a}^{-1}\right)$
and $R_{\chi,A_{m}',f_{a}^{-1}}$ are continuous in $a$.

With the same composition notation from \eqref{eq:composition}, we
consider the operator 
\begin{align}
\mathcal{L}_{f_{a}}^{-1}\widehat{A_{m}'}\mathcal{L}_{f_{a}}\widehat{A_{m}'}^{-1} & =\mathrm{Op}_{\chi}^{\mathrm{Pfl}}\left(\left(A_{m}\circ T^{*}f_{a}\right)\#_{\chi}A_{m}^{-1}\right)+\mathrm{Op}_{\chi}^{\mathrm{Pfl}}\left(E_{\chi,a}\right)+R_{a}\in\Psi_{\rho}^{0}\label{eq:Pa}
\end{align}
where $a\mapsto E_{\chi,a}\in\Psi_{\rho}^{-\left(2\rho-1\right)}$
and $a\mapsto R_{a}\in\Psi^{-\infty}$ are continuous. Define 
\begin{equation}
P_{a}:=\left(A_{m}\circ T^{*}f_{a}\right)\#_{\chi}A_{m}^{-1}+E_{\chi,a}.\label{eq:Pa_defin}
\end{equation}

We note that $\left\Vert \mathcal{L}_{f_{a}}\right\Vert _{H^{m}\to H^{m}}=\left\Vert \mathcal{L}_{f_{a}}^{-1}\widehat{A_{m}'}\mathcal{L}_{f_{a}}\widehat{A_{m}'}^{-1}\right\Vert _{L^{2}\to L^{2}}\sim\left\Vert \widehat{P_{a}}\right\Vert _{L^{2}\to L^{2}}$.
Since $\mathcal{L}_{f_{a}}$ on $H^{m}$ is the conjugate of $\widehat{A_{m}'}\mathcal{L}_{f_{a}}\widehat{A_{m}'}^{-1}$
on $L^{2}$ via the unitary map $\widehat{A_{m}'}:H^{m}\to L^{2}$,
all that remains is to decompose $\mathcal{L}_{f_{a}}\widehat{P_{a}}=\widehat{R_{a}}+\widehat{K_{a}}$where
\begin{align}
\left\Vert \widehat{R_{a}}\right\Vert _{L^{2}\to L^{2}} & \leq e^{-c_{3}p}\label{eq:contract_R}\\
\left\Vert \widehat{K_{a}}\right\Vert _{H^{s_{1}}\to H^{s_{2}}} & \lesssim_{s_{1},s_{2},\neg a}1\label{eq:uniform_smoothing-1}
\end{align}

Because of \eqref{eq:Pa_defin}, we know
\[
P_{a}-\frac{A_{m}\circ T^{*}f_{a}}{A_{m}}\in S_{\rho}^{-\left(2\rho-1\right)}
\]
Recall that based on how we defined $A_{m}$, we have 
\[
\left|\frac{A_{m}\circ T^{*}f_{a}}{A_{m}}\left(x,\xi\right)\right|\leq e^{-c_{2}p}\;\forall\left|\xi\right|_{g}\gtrsim_{\neg a}1
\]
 which implies 
\[
e^{-c_{2}p}-\left|P_{a}\left(x,\xi\right)\right|^{2}>0\;\forall\left|\xi\right|_{g}\gtrsim_{\neg a}1
\]
We then note that $e^{-c_{2}p}-\widehat{P_{a}}^{*}\widehat{P_{a}}\in\Psi_{\rho}^{0}$
is formally self-adjoint and elliptic. By Hormander's square root
trick, there is $b_{a}\in S_{1}^{0}$ such that 
\[
\widehat{L_{a}}:=e^{-c_{2}p}-\widehat{P_{a}}^{*}\widehat{P_{a}}-\widehat{b_{a}}^{*}\widehat{b_{a}}\in\Psi^{-\infty}
\]
Because taking the square root \eqref{eq:square_root_cont} and composition
is continuous, we can conclude $\left\Vert \widehat{L_{a}}\right\Vert _{H^{-1}\to L^{2}}\lesssim_{\neg a}1$.
Now we observe 
\[
\left\Vert \widehat{P_{a}}\phi\right\Vert _{L^{2}}^{2}\leq e^{-c_{2}p}\left\Vert \phi\right\Vert _{L^{2}}^{2}+\left\Vert \widehat{L_{a}}\phi\right\Vert _{L^{2}}\left\Vert \phi\right\Vert _{L^{2}}
\]
which implies that $\forall N\geq1$:
\begin{align*}
\left\Vert \widehat{P_{a}}P_{>N}\phi\right\Vert _{L^{2}}^{2} & \leq e^{-c_{2}p}\left\Vert P_{>N}\phi\right\Vert _{L^{2}}^{2}+\left\Vert \widehat{L_{a}}P_{>N}\phi\right\Vert _{L^{2}}\left\Vert P_{>N}\phi\right\Vert _{L^{2}}\\
 & \leq e^{-c_{2}p}\left\Vert \phi\right\Vert _{L^{2}}^{2}+\frac{1}{N}\left\Vert \widehat{L_{a}}\right\Vert _{H^{-1}\to L^{2}}\left\Vert \phi\right\Vert _{L^{2}}^{2}\leq\left(e^{-c_{2}p}+\frac{C}{N}\right)\left\Vert \phi\right\Vert _{L^{2}}^{2}
\end{align*}
where $C$ does not depend on small $a$.

There is $N_{0}\left(c_{2},p\right)$ such that $\forall N\geq N_{0}\left(c_{2},p\right):\left\Vert \widehat{P_{a}}P_{>N}\phi\right\Vert _{L^{2}}^{2}\leq e^{-\frac{1}{2}c_{2}p}\left\Vert \phi\right\Vert _{L^{2}}^{2}$.
Then we can simply define 
\[
\mathcal{L}_{f_{a}}\widehat{P_{a}}=\underbrace{\mathcal{L}_{f_{a}}\widehat{P_{a}}P_{>N_{0}}}_{=:\widehat{R_{a}}}+\underbrace{\mathcal{L}_{f_{a}}\widehat{P_{a}}P_{\leq N_{0}}}_{=:\widehat{K_{a}}}
\]
So we obtain \eqref{eq:contract_R}. Since $P_{a}$ is defined in
\ref{eq:Pa_defin} with all terms continuous in $a$, and $P_{\leq N_{0}}$
has a smoothing effect, we obtain \eqref{eq:uniform_smoothing-1}.
\end{proof}



